How to Compute Modulo Prime-Power Sums

The problem of computing modulo prime-power sums is investigated in distributed source coding as well as computation over Multiple-Access Channel (MAC). We build upon group codes and present a new class of codes called Quasi Group Codes (QGC). A QGC is a subset of a group code. These codes are not closed under the group addition. We investigate some properties of QGC's, and provide a packing and a covering bound. Next, we use these bounds to derived achievable rates for distributed source coding as well as computation over MAC. We show that strict improvements over the previously known schemes can be obtained using QGC's.

==> MATH_template.tex <==
\usepackage{tikz}
%\usepackage{mathdots}
\usepackage[utf8]{inputenc}
%\usepackage[ margin=1in ]{geometry}

\usepackage{amsmath} \usepackage{amsthm} \usepackage{amsfonts} \usepackage{amssymb} 
\usepackage{epstopdf}
%\usepackage{mathtools}
\usepackage{graphicx}
%\usepackage{relsize}
%\usepackage{xy}
\input{xypic}
\usepackage{bbm}
%\setlength{\footskip}{20pt}

\usepackage{enumerate}

%\onecolumn

%\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lem}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}

\theoremstyle{definition}
\newtheorem{example}{Example}
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question}
\newtheorem{problem}{Problem}
\newtheorem*{prob*}{Problem}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{rems}{Remarks}
\newtheorem{para}{}
\newtheorem{summary}{Summary}



\renewcommand{\Re}[1]{\ensuremath{\operatorname{Re}\left\{#1\right\}}}
\renewcommand{\Im}[1]{\ensuremath{\operatorname{Im}\left\{#1\right\}}}

\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}

\global\long\def\Z{\mathrm{{\bf Z}}}
\global\long\def\N{\mathrm{{\bf N}}}
\global\long\def\Gal{\mathrm{Gal}}





\global\long\def\RR{\mathbb{R}}
\global\long\def\CC{\mathbb{C}}
\global\long\def\NN{\mathbb{N}}
\global\long\def\QQ{\mathbb{Q}}
\global\long\def\ZZ{\mathbb{Z}}
\global\long\def\EE{\mathbb{E}}
\global\long\def\PP{\mathbb{P}}
\global\long\def\FF{\mathbb{F}}

 \global\long\def\dd{\cdots}
\global\long\def\normal{\triangleleft}

\newcommand*{\Scale}[2][4]{\scalebox{#1}{\ensuremath{#2}}}%
